Data-driven particle dynamics: Structure-preserving coarse-graining for emergent behavior in non-equilibrium systems

Multiscale systems are ubiquitous in science and technology, but are notoriously challenging to simulate as short spatiotemporal scales must be appropriately linked to emergent bulk physics. When expensive high-dimensional dynamical systems are coarse-grained into low-dimensional models, the entropic loss of information leads to emergent physics which are dissipative, history-dependent, and stochastic. To machine learn coarse-grained dynamics from time-series observations of particle trajectories, we propose a framework using the metriplectic bracket formalism that preserves these properties by construction; most notably, the framework guarantees discrete notions of the first and second laws of thermodynamics, conservation of momentum, and a discrete fluctuation-dissipation balance crucial for capturing non-equilibrium statistics. We introduce the mathematical framework abstractly before specializing to a particle discretization. As labels are generally unavailable for entropic state variables, we introduce a novel self-supervised learning strategy to identify emergent structural variables. We validate the method on benchmark systems and demonstrate its utility on two challenging examples: (1) coarse-graining star polymers at challenging levels of coarse-graining while preserving non-equilibrium statistics, and (2) learning models from high-speed video of colloidal suspensions that capture coupling between local rearrangement events and emergent stochastic dynamics. We provide open-source implementations in both PyTorch and LAMMPS, enabling large-scale inference and extensibility to diverse particle-based systems.

==> header.tex <==

\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{authblk}
\usepackage{arxiv}

% Macros
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\nexp}[1]{\cdot 10^{#1}}
\newcommand{\dpar}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\diff}[2]{\frac{d #1}{d #2}}
\newcommand{\ddiff}[2]{\frac{\mathsf{D} #1}{\mathsf{D} #2}}
\newcommand{\Grad}{\nabla}

\newcommand{\mysecref}[1]{Section~\ref{#1}}
\newcommand{\myappref}[1]{Appendix~\ref{#1}}
\newcommand{\myeqref}[1]{Eq.~\eqref{#1}}
\newcommand{\myfigref}[1]{Fig.~\ref{#1}}
\newcommand{\myalgref}[1]{Algorithm~\ref{#1}}
\newcommand{\mytabref}[1]{Table~\ref{#1}}
\newcommand{\mytheoremref}[1]{Theorem~\ref{#1}}
\newcommand{\mypropref}[1]{Proposition~\ref{#1}}
\newcommand{\mylemmaref}[1]{Lemma~\ref{#1}}


% General Packages
\usepackage{url}
\usepackage{pgfplots}
\usepackage{algorithm,algpseudocode}
\usepackage{algorithmicx}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{gensymb}
\usepackage{siunitx}
\usepackage[colorlinks,bookmarksnumbered,bookmarksopen,citecolor=blue,urlcolor=blue,linkcolor=blue,]{hyperref}
%\usepackage{xcolor}
%\usepackage{subcaption}
%\usepackage{graphicx}
\usepackage{amsthm}
\usepackage{booktabs}

% enumerate and itemize spacing
\usepackage{enumitem}
\setlist[itemize]{leftmargin=2em}
\setlist[enumerate]{leftmargin=2em}

% Theorems
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{proposition}{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
%\theoremstyle{remark} % Defines the style
\newtheorem*{remark}{Remark} % Define an unnumbered Remark environment

% Transpose operator
\DeclareMathOperator{\tr}{tr}

% Only number equations if used
\usepackage{mathtools}
\mathtoolsset{showonlyrefs=true}
\usepackage{autonum}

% Stretch vertical arrays
%\renewcommand{\arraystretch}{1.5}

% Allow equation breaks between pages
\allowdisplaybreaks

% More colors
%\usepackage[dvipsnames]{xcolor}

% Table rule style
%\usepackage{booktabs}

% Reduce captions
%\usepackage{caption} 
%\captionsetup[table]{skip=5pt}

% Txt import plots
\usepackage{filecontents}

% Colors
\definecolor{tabblue}{HTML}{1f77b4}
\definecolor{taborange}{HTML}{ff7f0e}

\usepackage[scaled]{helvet}


==> plots/results_solids/results_solids.tex <==


\begin{tikzpicture}
\pgfplotsset{width=0.5*\textwidth, height=8cm}

\begin{axis}[
    %xlabel=$t$,
    width=0.5*\textwidth,
    height=4cm,
    ylabel=RDF,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1.5em}, % Adjust ylabel position
]
\addplot [color=black, thick, dashed] table[x=r_RDF, y=RDF_gt] {plots/results_solids/viscoelastic.txt};
\addplot [color=tabblue, thick] table[x=r_RDF, y=RDF_net] {plots/results_solids/viscoelastic.txt};
\legend{GT, Ours}
\end{axis}

        
        
\node[anchor=north west, font=\sffamily\bfseries\Large] at (-1,2.5) {A};
\node[anchor=north west, font=\sffamily\bfseries\Large] at (-1,-0.5) {B};   
        
             

\begin{axis}[
    xlabel=$r$,
    width=0.5*\textwidth,
    	yshift=-3.2cm,
    height=4cm,
    ylabel=RDF,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1.5em}, % Adjust ylabel position
    xlabel style={yshift=0.5em},
]
\addplot [color=black, thick, dashed] table[x=r_RDF, y=RDF_gt] {plots/results_solids/needle.txt};
\addplot [color=tabblue, thick] table[x=r_RDF, y=RDF_net] {plots/results_solids/needle.txt};
%\legend{GT, Ours}
\end{axis}



\end{tikzpicture}



==> plots/star_polymer/star_polymer.tex <==


\begin{tikzpicture}
\pgfplotsset{width=\textwidth, height=8cm}

\begin{axis}[
    %xlabel=$t$,
    width=0.33\textwidth,
    height=4cm,
    ylabel=VACF,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1.5em}, % Adjust ylabel position
    restrict y to domain*=0:0.3,
]
\addplot [color=black, thick, dashed] table[x=t_vec, y=VACF_gt] {plots/star_polymer/star_polymer_11.txt};
\addplot [color=tabblue, thick] table[x=t_vec, y=VACF_net] {plots/star_polymer/star_polymer_11.txt};
\legend{GT, Ours}
\end{axis}


\begin{axis}[xshift=0.33\textwidth,
    width=0.33\textwidth,
    height=4cm,
    %xlabel=$r$,
    ylabel=RDF,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1.5em}, % Adjust ylabel position
]
\addplot [color=black, thick, dashed] table[x=r_RDF, y=RDF_gt] {plots/star_polymer/star_polymer_11.txt};
\addplot [color=tabblue, thick] table[x=r_RDF, y=RDF_net] {plots/star_polymer/star_polymer_11.txt};
\end{axis}


\begin{axis}[xshift=0.66\textwidth,
    width=0.33\textwidth,
    height=4cm,
    %xlabel=$t$,
    ylabel=MSD,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1.5em}, % Adjust ylabel position
    restrict y to domain*=0:6,
]
\addplot [color=black, thick, dashed] table[x=t_vec, y=MSD_gt] {plots/star_polymer/star_polymer_11.txt};
\addplot [color=tabblue, thick] table[x=t_vec, y=MSD_net] {plots/star_polymer/star_polymer_11.txt};
\end{axis}
        
        
\node[anchor=north west, font=\sffamily\bfseries\Large] at (-1,2.5) {A};
\node[anchor=north west, font=\sffamily\bfseries\Large] at (-1,-0.5) {B};   
        
        
        

\begin{axis}[
    xlabel=$t$,
    width=0.33\textwidth,
    	yshift=-3.2cm,
    height=4cm,
    ylabel=VACF,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1.5em}, % Adjust ylabel position
    xlabel style={yshift=0.5em},
    restrict y to domain*=0:0.3,
]
\addplot [color=black, thick, dashed] table[x=t_vec, y=VACF_gt] {plots/star_polymer/star_polymer_51.txt};
\addplot [color=tabblue, thick] table[x=t_vec, y=VACF_net] {plots/star_polymer/star_polymer_51.txt};
%\legend{GT, Ours}
\end{axis}


\begin{axis}[xshift=0.33\textwidth,
	yshift=-3.2cm,
    width=0.33\textwidth,
    height=4cm,
    xlabel=$r$,
    ylabel=RDF,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1.5em}, % Adjust ylabel position
    xlabel style={yshift=0.5em},
]
\addplot [color=black, thick, dashed] table[x=r_RDF, y=RDF_gt] {plots/star_polymer/star_polymer_51.txt};
\addplot [color=tabblue, thick] table[x=r_RDF, y=RDF_net] {plots/star_polymer/star_polymer_51.txt};
\end{axis}


\begin{axis}[xshift=0.66\textwidth,
	yshift=-3.2cm,
    width=0.33\textwidth,
    height=4cm,
    xlabel=$t$,
    ylabel=MSD,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1.5em}, % Adjust ylabel position
    restrict y to domain*=0:6,
    xlabel style={yshift=0.5em},
]
\addplot [color=black, thick, dashed] table[x=t_vec, y=MSD_gt] {plots/star_polymer/star_polymer_51.txt};
\addplot [color=tabblue, thick] table[x=t_vec, y=MSD_net] {plots/star_polymer/star_polymer_51.txt};
\end{axis}        
        

\end{tikzpicture}



==> plots/star_polymer_11/star_polymer_11.tex <==

\begin{tikzpicture}
\pgfplotsset{width=\textwidth, height=6cm}

\begin{axis}[
    xlabel=$t$,
    width=0.33\textwidth,
    ylabel=VACF,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1em}, % Adjust ylabel position
    restrict y to domain*=0:0.3,
]
\addplot [color=black, thick, dashed] table[x=t_vec, y=VACF_gt] {plots/star_polymer_11/star_polymer_11.txt};
%\addplot [color=red, thick] table[x=t_vec, y=VACF_net] {plots/star_polymer_11/star_polymer_11_gns.txt};
%\addplot [color=green, thick] table[x=t_vec, y=VACF_net] {plots/star_polymer_11/star_polymer_11_gns_sde.txt};
\addplot [color=tabblue, thick] table[x=t_vec, y=VACF_net] {plots/star_polymer_11/star_polymer_11.txt};
\end{axis}


\begin{axis}[xshift=0.33\textwidth,
    width=0.33\textwidth,
    xlabel=$r$,
    ylabel=RDF,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1em}, % Adjust ylabel position
]
\addplot [color=black, thick, dashed] table[x=r_RDF, y=RDF_gt] {plots/star_polymer_11/star_polymer_11.txt};
%\addplot [color=red, thick] table[x=r_RDF, y=RDF_net] {plots/star_polymer_11/star_polymer_11_gns.txt};
%\addplot [color=green, thick] table[x=r_RDF, y=RDF_net] {plots/star_polymer_11/star_polymer_11_gns_sde.txt};
\addplot [color=tabblue, thick] table[x=r_RDF, y=RDF_net] {plots/star_polymer_11/star_polymer_11.txt};
\legend{GT, Ours}
\end{axis}


\begin{axis}[xshift=0.66\textwidth,
    width=0.33\textwidth,
    xlabel=$t$,
    ylabel=MSD,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1em}, % Adjust ylabel position
    restrict y to domain*=0:6,
]
\addplot [color=black, thick, dashed] table[x=t_vec, y=MSD_gt] {plots/star_polymer_11/star_polymer_11.txt};
%\addplot [color=red, thick] table[x=t_vec, y=MSD_net] {plots/star_polymer_11/star_polymer_11_gns.txt};
%\addplot [color=green, thick] table[x=t_vec, y=MSD_net] {plots/star_polymer_11/star_polymer_11_gns_sde.txt};
\addplot [color=tabblue, thick] table[x=t_vec, y=MSD_net] {plots/star_polymer_11/star_polymer_11.txt};
\end{axis}
        
\end{tikzpicture}



==> plots/star_polymer_51/star_polymer_51.tex <==

\begin{tikzpicture}
\pgfplotsset{width=\textwidth, height=6cm}

\begin{axis}[
    xlabel=$t$,
    width=0.33\textwidth,
    ylabel=VACF,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1em}, % Adjust ylabel position
    restrict y to domain*=0:0.07,
    legend style={font=\tiny}, % Set legend font to tiny
]
\addplot [color=black, thick, dashed] table[x=t_vec, y=VACF_gt] {plots/star_polymer_51/star_polymer_51.txt};
%\addplot [color=red, thick] table[x=t_vec, y=VACF_net] {plots/star_polymer_51/star_polymer_51_gns.txt};
%\addplot [color=green, thick] table[x=t_vec, y=VACF_net] {plots/star_polymer_51/star_polymer_51_gns_sde.txt};
\addplot [color=tabblue, thick] table[x=t_vec, y=VACF_net] {plots/star_polymer_51/star_polymer_51.txt};
\end{axis}


\begin{axis}[xshift=0.33\textwidth,
    width=0.33\textwidth,
    xlabel=$r$,
    ylabel=RDF,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1em}, % Adjust ylabel position
]
\addplot [color=black, thick, dashed] table[x=r_RDF, y=RDF_gt] {plots/star_polymer_51/star_polymer_51.txt};
%\addplot [color=red, thick] table[x=r_RDF, y=RDF_net] {plots/star_polymer_51/star_polymer_51_gns.txt};
%\addplot [color=green, thick] table[x=r_RDF, y=RDF_net] {plots/star_polymer_51/star_polymer_51_gns_sde.txt};
\addplot [color=tabblue, thick] table[x=r_RDF, y=RDF_net] {plots/star_polymer_51/star_polymer_51.txt};
\legend{GT, Ours}
\end{axis}


\begin{axis}[xshift=0.66\textwidth,
    width=0.33\textwidth,
    xlabel=$t$,
    ylabel=MSD,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1em}, % Adjust ylabel position
    restrict y to domain*=0:3.5,
]
\addplot [color=black, thick, dashed] table[x=t_vec, y=MSD_gt] {plots/star_polymer_51/star_polymer_51.txt};
%\addplot [color=red, thick] table[x=t_vec, y=MSD_net] {plots/star_polymer_51/star_polymer_51_gns.txt};
%\addplot [color=green, thick] table[x=t_vec, y=MSD_net] {plots/star_polymer_51/star_polymer_51_gns_sde.txt};
\addplot [color=tabblue, thick] table[x=t_vec, y=MSD_net] {plots/star_polymer_51/star_polymer_51.txt};
\end{axis}
        
\end{tikzpicture}



==> plots/taylor_green/taylor_green.tex <==

\begin{tikzpicture}
\pgfplotsset{width=\textwidth, height=6cm}

\begin{axis}[
    xlabel=$t$,
    width=0.33\textwidth,
    ylabel=VACF,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1em}, % Adjust ylabel position
    restrict y to domain*=0:4.5,
    legend style={font=\tiny}, % Set legend font to tiny
]
\addplot [color=black, thick, dashed] table[x=t_vec, y=VACF_gt] {plots/taylor_green/taylor_green.txt};
%\addplot [color=red, thick] table[x=t_vec, y=VACF_net] {plots/taylor_green/taylor_green_gns.txt};
%\addplot [color=green, thick] table[x=t_vec, y=VACF_net] {plots/taylor_green/taylor_green_gns_sde.txt};
\addplot [color=tabblue, thick] table[x=t_vec, y=VACF_net] {plots/taylor_green/taylor_green.txt};
\end{axis}


\begin{axis}[xshift=0.33\textwidth,
    width=0.33\textwidth,
    xlabel=$r$,
    ylabel=RDF,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1em}, % Adjust ylabel position
    legend style={at={(0.95,0.05)},anchor=south east} % Legend in southeast
]
\addplot [color=black, thick, dashed] table[x=r_RDF, y=RDF_gt] {plots/taylor_green/taylor_green.txt};
%\addplot [color=red, thick] table[x=r_RDF, y=RDF_net] {plots/taylor_green/taylor_green_gns.txt};
%\addplot [color=green, thick] table[x=r_RDF, y=RDF_net] {plots/taylor_green/taylor_green_gns_sde.txt};
\addplot [color=tabblue, thick] table[x=r_RDF, y=RDF_net] {plots/taylor_green/taylor_green.txt};
\legend{GT, Ours}
\end{axis}


\begin{axis}[xshift=0.66\textwidth,
    width=0.33\textwidth,
    xlabel=$t$,
    ylabel=MSD,
    grid=major, % Display a grid
    grid style={dashed,gray!30}, % Set the style
    tick label style={font=\tiny}, % Smaller tick labels
    font=\small,
    ylabel style={align=center, yshift=-1em}, % Adjust ylabel position
    restrict y to domain*=0:0.65,
]
\addplot [color=black, thick, dashed] table[x=t_vec, y=MSD_gt] {plots/taylor_green/taylor_green.txt};
%\addplot [color=red, thick] table[x=t_vec, y=MSD_net] {plots/taylor_green/taylor_green_gns.txt};
%\addplot [color=green, thick] table[x=t_vec, y=MSD_net] {plots/taylor_green/taylor_green_gns_sde.txt};
\addplot [color=tabblue, thick] table[x=t_vec, y=MSD_net] {plots/taylor_green/taylor_green.txt};
\end{axis}
        
\end{tikzpicture}


